Peer Influence on West Point Cadets' Civil War Allegiances

Do social networks and peer influence shape major life decisions in highly polarized settings? We explore this question by examining how peers influenced the allegiances of West Point cadets during the American Civil War. Leveraging quasi-random variations in the proportion of cadets from Free States, we analyze how cadets' decisions about which army to join depended on the composition of their peers. We have three main findings. First, there was a strong and significant peer effect: a higher proportion of classmates from Free States significantly increased the likelihood that cadets from Slave States joined the Union Army. Second, the peer effect varies with geography, most notably with the slave population share in cadets' home states or counties, and with cadets' own slave ownership in 1860. Third, peer effects were amplified by shared experiences such as having served together in the Mexican-American War, continuous military service, and belonging to the same cohort, suggesting that sustained interaction is important.

==> A_PreambleSettings.tex <==


%%%%%%%%% Times New Roman Font %%%%%%%%%%%%%%%%%%%%
\usepackage{amsthm}
\usepackage{newtxtext,newtxmath} % Use Times New Roman font for text and math

%\usepackage[pdftex, colorlinks=true, citecolor =true]{hyperref} % This package makes the section numbers red.

%%%%%%%% Set Page Margins using geometry %%%%%%%%%%%%%%%%%%%%
\RequirePackage[
left=1in,
right=1in,
top=1in,
bottom=1in,
headheight=0pt,
headsep=0pt]{geometry}

%%%%%%%% Line Spacing %%%%%%%%%%%%%%%%%%%%
\setlength{\headsep}{5pt} % Set the distance between the header and the body text

\linespread{1.35} % Set the line spacing to 1.35 times the normal spacing

\RequirePackage[shortlabels,inline]{enumitem} % Customize lists with inline labels
\setlist{nolistsep} % Remove extra vertical spacing between items in lists



%%%%%%%% Figure %%%%%%%%%%%%%%%%%%%%
\usepackage{graphicx}
\graphicspath{{Figures/}}
\usepackage{subfig}
\captionsetup[subfigure]{width=0.8\textwidth}
%\usepackage{subcaption}
\usepackage{caption}

\usepackage{tikz} % Package for creating graphics with TikZ
\usetikzlibrary{calc} % Load additional TikZ libraries


%%%%%%%% Table %%%%%%%%%%%%%%%%%%%%
\usepackage{booktabs} % Package for better-looking tables
\usepackage{threeparttable} % Package for adding notes to tables



%%%%%%%% Captions of Figures and Tables %%%%%%%%%%%%%%%%%%%%
\RequirePackage[font=small,labelfont={bf}]{caption} % Customize caption font and format
\captionsetup[table]{skip=3pt} % Set skip space for table captions
\captionsetup[figure]{skip=3pt} % Set skip space for figure captions


%%%%%%%% Math %%%%%%%%%%%%%%%%%%%%
\usepackage{amssymb,latexsym,verbatim,layout,enumerate} % Packages for mathematical symbols, theorems, etc.
\usepackage{amsmath} % Package for advanced mathematical typesetting
%\usepackage{commath} % Uncomment this line if you need to use the commath package
\DeclareMathOperator*{\argmin}{arg\,min} % Define a math operator for argmin
\DeclareMathOperator*{\argmax}{arg\,max} % Define a math operator for argmax
\DeclareMathOperator*{\plim}{plim} % Define a math operator for plim




%%%%%%%% Hyperlinks %%%%%%%%%%%%%%%%%%%%
\usepackage{hyperref} % Package for hyperlinks
\RequirePackage{xcolor} % Package for color definitions
\definecolor{winered}{rgb}{0.5,0,0} % Define a custom color
\hypersetup{colorlinks=true, linkcolor=blue, citecolor=blue, urlcolor=blue}
%\hypersetup{colorlinks,linkcolor={winered},citecolor={winered},urlcolor={winered}} % Set hyperlink colors
\usepackage{url} % Package for typesetting URLs




%%%%%%%%% References, Citation %%%%%%%%%%%%%%%%%%%%
% Requires chicago-ff.bst
\usepackage[sort&compress]{natbib}
%\usepackage[authoryear]{natbib}
\setlength{\bibsep}{0.0pt}
%\bibliographystyle{Reference/chicago-ff-adjust}
\setlength{\bibsep}{2.5pt}
%\usepackage[margin = 1in]{geometry}
%\RequirePackage[\ELEGANT@cite,sort&compress]{natbib}
%\setlength{\bibsep}{0.0pt}
\def\bibfont{\footnotesize}



%\graphicspath{{image/}{figure/}{fig/}{img/}}
\RequirePackage[font=small,labelfont={bf}]{caption}
\captionsetup[table]{skip=3pt}
\captionsetup[figure]{skip=3pt}

\RequirePackage[shortlabels,inline]{enumitem}
\setlist{nolistsep}


%%%%%%%%% Remove Part Numbering/Heading %%%%%%%%%%%%%%%%%%%%
\renewcommand \thepart{} % Remove part numbering
\renewcommand \partname{} % Remove part heading


\usepackage{pdfpages} % Package for including PDF pages
\usepackage{setspace} % Package for adjusting line spacing
\usepackage{pdflscape} % Package for landscape-oriented pages

\usepackage{caption}
\captionsetup{justification=centering}



\usepackage{minitoc}

\usepackage{parskip} % Disable paragraph indentation and add some vertical space between paragraphs
\renewcommand{\abstractname}{Abstract} % Rename the abstract heading
\newtheorem{theorem}{Theorem} % Define a theorem environment
\newtheorem{lemma}{Lemma} % Define a lemma environment
\newtheorem{proposition}{Proposition} % Define a proposition environment
\newtheorem{corollary}{Corollary} % Define a corollary environment
\newtheorem{assumption}{Assumption} % Define an assumption environment
\newtheorem{hypothesis}{Hypothesis} % Define a hypothesis environment
\renewcommand \thepart{} % Remove part numbering
\renewcommand \partname{} % Remove part heading
\usepackage{pdfpages} % Package for including PDF pages
\usepackage{setspace} % Package for adjusting line spacing
\usepackage{pdflscape} % Package for landscape-oriented pages
\usepackage{afterpage} % Package for typesetting text after the current page
\usepackage{float} % Package for placing floats exactly

